Renormalization group theory for fermions and order parameter fluctuations in interacting Fermi systems

In this thesis, we perform a comprehensive renormalization group analysis of two- and three-dimensional Fermi systems at low and zero temperature. We examine systems with spontaneous symmetry-breaking and quantum critical behavior by deriving and solving flow equations within the functional renormalization group framework. We extend the Hertz-Millis theory of quantum phase transitions in itinerant fermion systems to phases with discrete and continuous symmetry-breaking, and to quantum critical points where the zero temperature theory is associated with a non-Gaussian fixed point. We compute the finite temperature phase boundary near the quantum critical point explicitly including non-Gaussian fluctuations. We then set up a coupled fermion-boson renormalization group theory that captures the mutual interplay of gapless fermions with massless order parameter fluctuations when approaching a quantum critical point. As a first application, we compute the complete set of quantum critical exponents at the semimetal-to-superfluid quantum phase transition of attractively interacting Dirac fermions in two dimensions. Both, the order parameter propagator and the fermion propagator become non-analytic functions of momenta destroying the Fermi liquid behavior. We finally compute the effects of quantum fluctuations in the superfluid ground state of an attractively interacting Fermi system, employing the attractive Hubbard model as a prototype. The flow equations capture the influence of longitudinal and Goldstone order parameter fluctuations on non-universal quantities such as the fermionic gap and the fermion-boson vertex, as well as the exact universal infrared asymptotics present in every fermionic superfluid.

==> KT_finiteT.tex <==


\chapter[Kosterlitz-Thouless phase of fermionic superfluids at finite temperature]{Kosterlitz-Thouless phase of fermionic superfluids at finite temperature}
\label{chap:KT}


\section{Introduction}


\subsection{Continuum Model}
%
In this chapter, we consider the lattice dispersion (see Fig.\ref{fig:fs}) in the limit of 
low band-filling, where the Fermi surface becomes spherically symmetric and it 
resembles the continuum model and is well approximated by the dispersion,
%
\begin{eqnarray}
\xi_{\mathbf{k}}=\mathbf{k}^{2}-\mu\;,
\end{eqnarray}
%
with the effective fermion mass set to unity.



\section{RG Truncation}
%
We here utilize optimized Litim cutoffs (Litim 2001) for spatial momenta for 
fermions,
%
\begin{eqnarray}
R_{f\Lambda}\left(\xi_{\mathbf{k}}\right)&=&
Z_{f}\left(-\Lambda_{f}\,\text{sgn}\left[\xi_{\mathbf{k}}\right]
+ \xi_{\mathbf{k}}\right)
\theta\left[\Lambda_{f} - |\xi_{\mathbf{k}}|\right]\;,
\end{eqnarray}
%
which replaces the Fermi dispersion with a constant for momentum-modes 
closer to the Fermi surface than $\Lambda_{f}(\Lambda)$ and $Z_{f}$ denotes the fermionic 
field renormalization. Importantly, this choice of cutoff for spatial momenta does not 
affect analyticity properties of the fermion Green function in the complex (frequency) plane. 
Moreover, the fermion propagator remains fully differentiable with respect to frequency.

The bosonic excitations are split into a longitudinal mode $\sigma$ and a massless 
Goldstone mode $\pi$ for which we employ,
%
\begin{eqnarray}
R_{\sigma\Lambda}(\mathbf{q})&=&Z_{\sigma}\left(\Lambda_{\sigma}^{2} -
\mathbf{q}^{2}\right) \theta\left[\Lambda_{\sigma}^{2} -
\mathbf{q}^{2}\right]
\nonumber\\
R_{\pi\Lambda}(\mathbf{q})&=&Z_{\sigma}\left(\Lambda_{\pi}^{2} -
\mathbf{q}^{2}\right) \theta\left[\Lambda_{\pi}^{2} -
\mathbf{q}^{2}\right]\;,
\label{eq:kt_bose_cutoffs}
\end{eqnarray}
%
where $Z_{\sigma}$ and $Z_{\pi}$ are the corresponding field renormalizations factors.
%

\subsection{Fermion self-energy}
%
In two dimensions at finite temperature, diagrams containing any single Goldstone propagator 
exhibit logarithmic divergences for small momenta. Therefore, the diagrams renormalizing 
the normal component of the fermion self-energy depicted in Fig. \ref{fig:kt_fermionic_self} 
potentially lead to singular corrections to the fermionic self-energy.

\begin{figure}[b]
\begin{fmffile}{20080909_ferm_normal_4}
\begin{eqnarray}
Z_{f},\,\,A_{f}&:&
\parbox{45mm}{\unitlength=1mm\fmfframe(2,2)(1,1){
\begin{fmfgraph*}(42,35)\fmfpen{thin} %pp-with rpa with ladder,  inset
\fmfleft{l1}
 \fmfright{r1}
 \fmfpolyn{hatched,tension=0.4}{G}{3}
 \fmfpolyn{hatched,tension=0.4}{K}{3}
  \fmf{fermion}{l1,G1}
   \fmf{fermion,straight,tension=0.5,left=0.}{K3,G2}
  \fmf{dashes,tension=0.,left=0.7}{G3,K2}
  \fmf{fermion}{K1,r1}
 \end{fmfgraph*}
}}
\hspace{3mm}
 + 
\hspace{3mm}
\parbox{45mm}{\unitlength=1mm\fmfframe(2,2)(1,1){
\begin{fmfgraph*}(42,35)\fmfpen{thin} %pp-with rpa with ladder,  inset
\fmfleft{l1}
 \fmfright{r1}
 \fmfpolyn{filled=30,tension=0.4}{G}{3}
 \fmfpolyn{filled=30,tension=0.4}{K}{3}
  \fmf{fermion}{l1,G1}
   \fmf{fermion,straight,tension=0.5,left=0.}{K3,G2}
  \fmf{photon,tension=0.,right=0.7}{K2,G3}
  \fmf{fermion}{K1,r1}
 \end{fmfgraph*}
}}\nonumber\\[-20mm]
%
\nonumber
\end{eqnarray}
\end{fmffile}
\caption{Contribution to the normal fermion self-energy 
below $\Lambda_{c}$.}
\label{fig:kt_fermionic_self}
\end{figure}


To investigate this further, we use in a first step for the fermion quadratic term in the 
effective action the ansatz
%
\begin{equation}
 \Gam_{\psib\psi} = - \int_{k\sg} 
 \psib_{k\sg} Z_f(\, ik_0 - \, \xi_{\bk}) \, 
 \psi_{k\sg} \; ,
\end{equation}
%
with cutoff-dependent renormalization factor $Z_f$. 
This corresponds to a propagator describing fermionic
quasiparticles with a reduced spectral weight $1/Z_f$:
%
\begin{eqnarray}
G_{f}(k)=\frac{Z_{f}^{-1}}{ik_{0}-\xi_{\mathbf{k}}}\,\,. 
\end{eqnarray}
%
The initial condition for the flow of $Z_f$ can be read off 
from the bare action as $Z_f = 1$.

The anomalous term is modified by the presence of the fermionic 
field renormalization and reads 
%
\begin{equation}
 \Gam_{\psi\psi} = Z_f \int_k \left(
 \Delta \, \psib_{-k\down} \psib_{k\up} + 
 \Delta^* \psi_{k\up} \psi_{-k\down} \right)\;.
\end{equation}
%
The normal and anomalous fermionic propagators corresponding
to $\Gam_{\psib\psi}$ and $\Gam_{\psi\psi}$ have the form
%
\begin{eqnarray}
 G_f(k) &=& Z_f^{-1} \,
 \frac{-ik_0 - \xi_{\bk}}{k_0^2 + E_{\bk}^2}
 \\
 F_f(k) &=& Z_f^{-1} \,
 \frac{\Delta}{k_0^2 + E_{\bk}^2} \; ,
\end{eqnarray}
%
where $E_{\bk} = (\xi_{\bk}^2 + |\Delta|^2 )^{1/2}$.

The flow equation for $Z_{f}$ in the symmetry-broken phase is given by
%
\begin{equation}
 \partial_{\Lam} Z_f = \int_{q, R_{s}} \partial_{ik_0}
 \left. G_f(q-k) \, [g^2_{\sg} G_{\sg}(q) + g^2_{\pi} G_{\pi}(q)]
 \right|_{k=(0,\bk_F)}\;,
\end{equation}
%
and accordingly the left-hand-side of the flow equation for $\Delta$ 
receives an additional factor of $Z_{f}$\;,
%
\begin{equation}
 \partial_{\Lam} (Z_f \Delta) = 
 g_{\sg} \, \partial_{\Lam} \alf
 - \! \int_{q, R_{s}} \! \left. F_f(q-k) \, 
 [g^2_{\sg}G_{\sg}(q) - g^2_{\pi}G_{\pi}(q)] \right|_{k=(0,\bk_F)} \; .
\end{equation}
%
%

\section{Infrared asymptotics}
%
In the regime $\Lam\rightarrow 0$, the bosonic sector is driven by the classical 
zeroth Matsubara frequency. The Matsubara summation splits into a classical 
and quantum part
%
\begin{eqnarray}
T\sum_{\Omega_{n}}=T\sum_{\Omega_{n}=0}^{(\text{class})}
+T\sum_{\Omega_{n}\neq 0}^{(\text{quant})}\;,
\end{eqnarray}
%
where $\Omega_{n}=2\pi n T$ is the bosonic Matsubara frequency, with $n$ integer. 
The purely fermionic summations do not contribute in the infrared as they are regularized 
by the lowest Matsubara frequency $~ \pi T$ (``thermal mass``). In mixed diagrams, the fermion 
propagators are evaluated at $\omega_{n}=\pi T$.

\subsection{Bosonic sector}

In terms of variables, it is convenient to define
%
\begin{eqnarray}
\tilde{\lambda}&=&\frac{\lambda}{Z_{\sigma}^{2}\Lambda^{2}}\nonumber\\
\tilde{\alpha}^{2}&=&Z_{\sigma}\alpha^{2}\nonumber\\
\tilde{Z}_{\pi}&=&\frac{Z_{\pi}}{Z_{\sigma}}\;,
\end{eqnarray}
%
where $\tilde{\alpha}^{2}$ denotes the square of the renormalized order-parameter 
and can be associated with the superfluid density $\tilde{\rho}$. Defining further 
the anomalous dimensions for the $\sigma$- and $\pi$-field,
%
\begin{eqnarray}
\eta_{Z_{\sigma}}&=&- \frac{d \log Z_{\sigma}}{d\log \Lambda}\nonumber\\
\eta_{Z_{\pi}}&=&- \frac{d \log Z_{\pi}}{d\log \Lambda}\,\,,
\end{eqnarray}
%
the flow equations for the superfluid density and the quartic coupling can be written as
%
\begin{eqnarray}
\frac{d \tilde{\rho}}{d\log\Lam}&=&-\eta_{\sigma}\tilde{\rho}
+
\frac{T}{2\pi}\left[
\frac{3}{\left(1+\tilde{\lambda}\tilde{\rho}\right)^{2}}
+
\frac{1}{\tilde{Z}_{\pi}}
\right]
\nonumber\\
%
\frac{d \tilde{\lambda}}{d\log\Lam}&=&\left(2\eta_{\sigma}-2\right)\tilde{\lambda}
+
\frac{T}{\pi}\tilde{\lambda}^{2}
\left[
\frac{9}{\left(1+\tilde{\lambda}\tilde{\rho}\right)^{3}}
+
\frac{1}{\tilde{Z}_{\pi}^{2}}
\right]\;.
\end{eqnarray}
%
The anomalous dimensions are determined by
%
%
\begin{eqnarray}
\eta_{\sigma}&=&\frac{T}{2\pi} 3\tilde{\lambda}^{2}\tilde{\rho}
\left[
\frac{3}{\left(1+\tilde{\lambda}\tilde{\rho}\right)^{4}}
+
\frac{1}{\tilde{Z}^{3}_{\pi}}
\right]\nonumber\\
%
\eta_{\pi}&=&\frac{T}{\pi} \frac{\tilde{\lambda}^{2}\tilde{\rho}}
{\tilde{Z}^{2}_{\pi}}
\left[
\frac{2}{1+\tilde{\lambda}\tilde{\rho}}
+
\frac{1}{\left(1+\tilde{\lambda}\tilde{\rho}\right)^{2}}\right]\nonumber\\
%
\frac{d \tilde{Z}_{\pi}}{d\log\Lam}&=&
\left(\eta_{\sigma}-\eta_{\pi}\right)
\tilde{Z}_{\pi}\;.
\end{eqnarray}
%
Different flow equations accounting for only one bosonic mode in the Kosterlitz-Thouless phase 
have been presented in (Gr\"ater 1995, v. Gersdorff 2001, Berges 2002).



%
\subsection{Fermi-Bose sector}
%
Order-parameter fluctuations represented by the Goldstone and longitudinal mode couple back 
into the fermionic sector of the system by the diagrams depicted in Fig. \ref{fig:kt_fermionic_self} for the normal self-energy, Fig. \ref{fig:fermionic_self} for the anomalous self-energy and 
Fig. \ref{fig:vertex_ssb} for the fermion-boson vertex.

To this end, we define for the fermion-boson vertices the rescaled variables and fermion anomalous 
dimension
%
\begin{eqnarray}
\tilde{g}^{2}_{\sigma}&=&\frac{g_{\sigma}^{2}}{Z_{f}^{2}\, Z_{\sigma}}\nonumber\\
\tilde{g}^{2}_{\pi}&=&\frac{g_{\pi}^{2}}{Z_{f}^{2}\, Z_{\sigma}}\nonumber\\
\eta_{f}&=&- \frac{d \log Z_{f}}{d\log \Lambda}\;,
\end{eqnarray}
%
in terms of which we write the flow equations for the fermion gap and anomalous 
dimension
%
\begin{eqnarray}
\frac{d \Delta}{d \log \Lambda}&=& \eta_{f} \Delta + 
\frac{\tilde{g}_{\sigma}}{2\sqrt{\tilde{\rho}}}\left(\frac{d \tilde\rho}{d \log \Lambda}
+ \eta_{\sigma} \tilde{\rho}\right)
+
\frac{T}{2\pi}\left(\frac{\Delta}{\left(\pi T\right)^{2} +|\Delta|^{2}}
\left[
\frac{\tilde{g}_{\sigma}^{2}}{\left(1+\tilde{\lambda}\tilde{\rho}\right)^{2}}
-
\frac{\tilde{g}_{\pi}^{2}}{\tilde{Z}_{\pi}}
\right]
\right)\nonumber\\
%
\eta_{f}&=& \frac{T}{2\pi}\frac{1}{\left(\pi T \right)^{2} + |\Delta|^{2}}
\left[
\frac{\tilde{g}_{\sigma}^{2}}{\left(1+\tilde{\lambda}\tilde{\rho}\right)^{2}}
+
\frac{\tilde{g}_{\pi}^{2}}{\tilde{Z}_{\pi}}
\right]\;.
\end{eqnarray}
%
The fermion-boson vertices evolve in accordance with
%
\begin{eqnarray}
\frac{d \tilde{g}_{\sigma}}{d \log \Lambda}&=&
\left(\eta_{f}+\frac{1}{2}\eta_{\sigma}\right)\tilde{g}_{\sigma}
+
\frac{T}{2\pi}\tilde{g}_{\sigma}\left(
\frac{|\Delta|^{2}-\left(\pi T\right)^{2}}
{\left(\pi T\right)^{2} +|\Delta|^{2}}
\left[
\frac{\tilde{g}_{\pi}^{2}}{\tilde{Z}_{\pi}}
-
\frac{\tilde{g}_{\sigma}^{2}}{\left(1+\tilde{\lambda}\tilde{\rho}\right)^{2}}
\right]
\right)
\nonumber\\
%
\frac{d \tilde{g}_{\pi}}{d \log \Lambda}&=&
\left(\eta_{f}+\frac{1}{2}\eta_{\sigma}\right)\tilde{g}_{\pi}
+
\frac{T}{2\pi}\tilde{g}_{\pi}\left(
\frac{1}
{\left(\pi T\right)^{2} +|\Delta|^{2}}
\left[
\frac{\tilde{g}_{\pi}^{2}}{\tilde{Z}_{\pi}}
-
\frac{\tilde{g}_{\sigma}^{2}}{\left(1+\tilde{\lambda}\tilde{\rho}\right)^{2}}
\right]
\right)\;.
\end{eqnarray}
%
The fermionic cutoff has been taken to zero by setting $\Lambda_{f}\rightarrow0$ as the fermionic 
propagators are regularized by their thermal mass $\pi T$ even for vanishing gaps.




\section{Energy gap in the single-particle spectrum}
\label{sec:spectral}

\subsection{Spectral function}

\subsection{Specific heat}

%
\section{Conclusion}
%


%


==> dedic.tex <==

%
\thispagestyle{empty}
\vspace*{3.5cm}
\begin{flushright}

% write your text here
{
\Large
Dedicated to Rolf-Dieter (1953--)\\
Elisabeth (1952--)\\
Anne Gerrit (1982--)\\
}
%\newpage
%\mbox{}
%\thispagestyle{empty}
%fuck up
%\cleardoublepage 
\end{flushright}


==> pref.tex <==

\preface

This Master's thesis has been submitted in partial fulfillment of
requirements for an advanced degree at The University of Arizona and
is deposited in the University Library to be made available to
borrowers under the rules of the Library.\vspace{3mm}

Brief quotations from this Master's thesis are allowable without
special permission, provided that an accurate acknowledgment of
source is made. Requests for permission for extended quotation from
or reproduction of this manuscript in whole or in part may be
granted by the copyright holder.\vspace{3mm}

\noindent SIGNED:\textit{Philipp Strack}\vspace{5mm}

\noindent APPROVAL BY THESIS DIRECTOR:\textit{Adam Burrows}
(Professor of Astronomy), 25 April 2005


==> summary_part2.tex <==
%
\chapter[Highlights Part II]{Highlights Part II}
%
We briefly highlight the main results obtained in this thesis.


%\section{Quantum Criticality}
%
%\section{Symmetry-breaking}
%












%

